Fixed Points of the Set-Based Bellman Operator

Motivated by uncertain parameters encountered in Markov decision processes (MDPs), we study the effect of parameter uncertainty on Bellman operator-based methods. Specifically, we consider a family of MDPs where the cost parameters are from a given compact set. We then define a Bellman operator acting on an input set of value functions to produce a new set of value functions as the output under all possible variations in the cost parameters. Finally we prove the existence of a fixed point of this set-based Bellman operator by showing that it is a contractive operator on a complete metric space.

==> IntervalMDP.tex <==
\section{Example}
\begin{figure}[h]
    \centering
    \includegraphics[width = 0.6\columnwidth]{fig/MDP_ex.png}
    \caption{2 state 2 action MDP }
    \label{fig:2S2A_MDP}
\end{figure}
Suppose we have a 2 state, 2 action MDP given by Figure~\ref{fig:2S2A_MDP}, whose cost and transition probabilities are given by Table~\ref{tab:2S2A_P}.
\begin{table}[h]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
& $(1, a_1)$ & $(1, a_2)$ & $(2, a_1)$ & $(2, a_2)$ \\ \midrule
$P_{1, (s,a)}$ & 0.9        & 0.1          & 0.9        & 0.5          \\
$P_{2, (s,a)}$ & 0.1        & 0.9          & 0.1        & 0.5          \\
$C_{s,a}$      & $4 \pm 0.6$          & $5  \pm 0.7$        & $3 \pm 0.5$    & $1 \pm 1$         \\ \bottomrule
\end{tabular}
\label{tab:2S2A_P}
\end{table}
The cost has uncertainty within the given bounds. We investigate using a couple different methods to calculate the value function bounds on this system. I.e. by using interval arithmetic, affine arithmetic, and Sarah's secret sauce arithmetic, apply value iteration and see where it takes me. 

For each of the three methods, we are mostly concerned with addition/subtraction of intervals, multiplication by a scalar, and minimization over a discrete set. 

\subsection{Interval Arithmetic}
Interval arithmetic follows these rules for the different operations. 
\begin{equation}
    \begin{aligned}
        [a, b] + [c, d] & = [a + c, b + d] \\
        [a, b] - [c, d] & = [a - c, b - d] \\
        \min\{[a, b], [c, d]\} &  = [\min\{a, c\}, \min\{b, d\}]
    \end{aligned}
\end{equation}
The cost uncertainties written in interval form is $C_{ii} = [\underline{C_{ii}}, \overline{C_{ii}}]$. 

\subsubsection{Zeroth iteration}
Going through value function iteration, the initial value function is given by
\begin{equation}
    \begin{aligned}
        V_0(1) & = \min\{[\underline{C_{11}}, \overline{C_{11}}], [\underline{C_{12}}, \overline{C_{12}}]\} \\
        V_0(2) & = \min\{[\underline{C_{21}}, \overline{C_{21}}], [\underline{C_{22}}, \overline{C_{22}}],\}
    \end{aligned}
\end{equation}

From interval arithmetics, 
\begin{equation}
    \begin{aligned}
        V_0(1) & = [\min\{\underline{C_{11}}, \underline{C_{12}}\}, \min\{\overline{C_{11}},  \overline{C_{12}}\}] \\
        V_0(2) & = [\min\{\underline{C_{21}}, \underline{C_{22}} \}, \min\{\overline{C_{21}}, \overline{C_{22}}\} ]
    \end{aligned}
\end{equation}

Let $\min\{\underline{C_{s1}}, \underline{C_{s2}}\} = \underline{V_0}(s)$ and  $\min\{\overline{C_{s1}}, \overline{C_{s2}}\} = \overline{V_0}(s)$, then the interval becomes 
\begin{equation}
    \begin{aligned}
        V_0(s) & = [\underline{V_0}(s),\overline{V_0}(s)]
    \end{aligned}
\end{equation}

\subsubsection{First iteration}
The first iteration is 
\[V_1(s)  = \min_{a} C_{sa} + P_{1sa}V_0(1) + P_{2sa}V_0(2),\]
Since each state has two actions, the minimization occurs over 2 distinct elements, i.e.
\[V_1(s) = \min\{ C_{s1} + P_{1s1}V_0(1) + P_{2s1}V_0(2), C_{s2} + P_{1s2}V_0(1) + P_{2s2}V_0(2)\}\]
However now we must treat each element as a set. The first element's interval is represented by 
\[[\underline{C_{s1}} + P_{1s1}\underline{V_0}(1) + P_{2s1}\underline{V_0}(2), \overline{C_{s1}} + P_{1s1}\overline{V_0}(1) + P_{2s1}\overline{V_0}(2)]\]
While the second element is represented by
\[[\underline{C_{s2}} + P_{1s2}\underline{V_0}(1) + P_{2s2}\underline{V_0}(2), \overline{C_{s2}} + P_{1s2}\overline{V_0}(1) + P_{2s2}\overline{V_0}(2)]\]
To obtain the interval representation of $V_1(s)$, which is the minimum over the two intervals given above, we skip a couple steps and get $V_1(s)$ is
\begin{align}
V_1(s) =  [&\min\{ &\underline{C_{s1}} + P_{1s1}\underline{V_0}(1) + P_{2s1}\underline{V_0}(2), \\
    &   &\underline{C_{s2}} + P_{1s2}\underline{V_0}(1) + P_{2s2}\underline{V_0}(2)\}, \\
    & \min \{&\overline{C_{s1}} + P_{1s1}\overline{V_0}(1) + P_{2s1}\overline{V_0}(2), \\
    &   &\overline{C_{s2}} + P_{1s2}\overline{V_0}(1) + P_{2s2}\overline{V_0}(2)\}]
\end{align}
Let
\begin{align}
\underline{V_1}(s) = \min\{& \underline{C_{s1}} + P_{1s1}\underline{V_0}(1) + P_{2s1}\underline{V_0}(2), \\ &\underline{C_{s2}} + P_{1s2}\underline{V_0}(1) + P_{2s2}\underline{V_0}(2)\}
\end{align}
and 
\begin{align}
\overline{V_1}(s) = \min \{&\overline{C_{s1}} + P_{1s1}\overline{V_0}(1) + P_{2s1}\overline{V_0}(2), \\
&\overline{C_{s2}} + P_{1s2}\overline{V_0}(1) + P_{2s2}\overline{V_0}(2)\}
\end{align}

Then $V_1(s) = [\underline{V_1}(s), \overline{V_1}(s)]$ holds.

Here we note that this far, each $\underline{V_i}(s)$ represents the lower bound of the possible value functions given uncertainty in cost function. However, through our derivation, it is obvious they are the results of taking value iteration over constant costs $\underline{C}$ for the lower bounds of the uncertainty in cost. Equivalently, $\overline{V_i}(s)$ represents the upper bound of the possible value functions given uncertainty in cost function; they are also the results of running precise value iteration on the upper bounds $\overline{C}$ of the cost function uncertainty. 

Based on this, the following theorem can be stated ( will prove at some point), 
\begin{theorem}
For an MDP with cost uncertainty given by $C \in [\underline{C}, \overline{C}]$, the value iteration algorithm returns, at the the $k^{th}$ step, a value function $V_k \in [\underline{V_k}, \overline{V_k}]$, where at each state, the upper and lower bounds are given by  
\begin{align}
\overline{V_k}(s) &  = \min_{a} \overline{C_{sa}} + \sum_{s'}P_{s'sa}\overline{V_{k-1}}(s) \\
\underline{V_k}(s) &  = \min_{a} \underline{C_{sa}} + \sum_{s'}P_{s'sa}\underline{V_{k-1}}(s) 
\end{align}
\end{theorem}

This is a fairly general result, it states that even if the costs are \emph{changing}, such that the resulting value iteration does \emph{not} converge, the value functions cannot leave the bounds given by $\underline{V_k}$ and $\overline{V_k}$. 

A natural consideration is, will value iteration also converge to the values given within these bounds? The answer is no. To see this, just consider when we choose $\underline{C} \in [\underline{C}, \overline{C}]$, the element that's the absolute lower bound. Because value iteration always returns an upper bound, we are guaranteed that $\underline{V}^\star \leq \underline{V}_k$ for all $k$. 

However when MDP is ergodic, we do have some sort of bound on $V_k$ for the mean average pay off case. 

==> Proposal.tex <==

\section{Bounding value approximation}
\label{sec:templates}

\ForAuthorsAssa{I will develop this part}
Given an input uncertain cost $\mc{C}$, we can outer approximate the output of $F_{\mc{C}}$ by a given template $h: \reals^S \rightarrow \reals^m$ and a bounding vector $\alpha_v \in \reals^m$ which satisfies 
\[F_{\mc{C}}(\mc{V}) \subseteq \Lambda = \{V \ | \ h(V) \leq \alpha_v\}\]
How closely $h(\mc{V}) \leq \alpha_v$ approximates $F_{\mc{C}}$ depends on both the template $h$ and the bounding vector $\alpha_v$. If the shape of $F_{\mc{C}}$ wildly differs the shape of $h$, then it's impossible to obtain a good approximation of $F_{\mc{C}}$. For the rest of this paper, we assume that $h$ is an \emph{affine function} in $V$, such that its sublevel sets are polytopes. Assuming that the given template $h$ can provide a good approximation, the quality of approximation then depends on $\alpha_v$.
\ForAuthorsAssa{By tight, you mean there is no $\alpha\in\reals^m$ such that $\{V\mid h(V)\leq \min (\alpha,\alpha_v)\}$ contains $F_{\mc{C}}(\mc{V})$?}
\tc{red}{yeah that sounds right}


\begin{proposition}
For each $j \in [m]$, approximating $F_{\mc{C}}(\mc{V})$ by $\Lambda  = \{V \ | \ h(V) \leq \alpha_v\} $ is tight if for each $j \in [m]$, 
\[\alpha_{vj} = \max_{C\in \Gamma, V \in \mc{V}}\  h_j(f_{C}(V))\]
\end{proposition}
\tc{blue}{As we said, we have to maximize on the closed convex hull of $F_{\mc{C}}(\mc{V})$ as $\Lambda$ is closed and convex.}
\begin{proof}
Two things: 1) that $F_{\mc{C}}(\mc{V}) \subseteq \Lambda$. This can be shown with the hyperplane separation theorem. 2) that for any $\alpha < \alpha_v$, the set $\Lambda$ will not contain $F_{\mc{C}}(\mc{V})$. This probably can also be shown with the hyperplane separation theorem. 
\end{proof}

\tc{blue}{I do not understand the proof. The maximizer $V^*$ of $h$ does not satisfy $V\leq V^*$ for all $V\in\mc{V}$. Then $f_C(V^*)$ is not necessarily better than $f_C(V)$ for all $V\in\mc{V}$. For example, take $h(x,y)=x-y$, $\mc{V}=[-10;10]\times [-5,5]$ and $f(x,y)=(\min(x,y),\max(x,y))$. The maximizer $V^*$ of $h$ on $\mc{V}$ is $(10,-5)$. Then $h(f(V^*))=\min(10,-5)-\max(10,-5)=-15$. However $\max_{(x,y)\in \mc{V}} h(f(x,y))\geq h(f(0,0))=0$.}

\tc{blue}{The aim of the theorem is to construct an algorithm to compute a representation of $F_\mc{C}(\mc{V})$ and for a given $h$ how to compute the value $\alpha$. }
\tc{red}{Hi Assale, this proposition should not hold for any general $F$, it should hold for just the bellman operator $F_{\mc{C}}$, which is an order preserving operator. We can talk about it tomorrow. This is basically my understanding of what you wrote on the board when we talked in Toulouse. }
\begin{theorem}
If $F_\mc{C}(\cdot)$ is an order preserving operation, each approximation $\Tilde{\Lambda}$ is determined by its coefficient and can be solved as 
\begin{align}
    \alpha_v &  =  \underset{C \in \Gamma, V\in\mc{V}}{\max } \ h(f_{C}(V))\\
    &  = \max_{C\in \Gamma}h\circ f_{C}\Big(\argmax_{V\in\mc{V}}h(V)\Big) \\
    % &  = h\circ \max_{C\in \Gamma}f_{C}\Big(\argmax_{V\in\mc{V}}h(V)\Big) \\
    &  = h\circ f_{C^\star}\Big(V^\star\Big) 
\end{align}
where $V^\star = \argmax_{V\in\mc{V}}h_j(V)$, and $C^\star = \argmax_{C \in\Gamma}h_j(f_{C}(V^\star))$
\end{theorem}
\
\ForAuthorsAssa{In the case where $x\mapsto h(x)=-x_i$, $h$ is not order-preserving. However, $-h$ is order-preserving and then $\max h=-\min -h$ and then we can extend the result to the min and we have $\max h=-F(z,-h(\argmin_{C\in\Gamma} C)$  }
\begin{proof}
Given $V$ and uncertainty set $\Gamma$, the output value functions are defined by 
\[F_{\mc{C}}(\mc{V}) = \{ V^+ \ | \ \exists\ C\in \Gamma, \ V\in \mc{V}, \ \text{ s.t. } V^+ = f_{C}(V)\}\]

We consider using generic template $h$ to over-approximate $F_{\mc{C}}(\mc{V})$. From Proposition 1, 
\[\alpha =  \underset{C \in \Gamma, V \in \mc{V}}{\max }\  h(f_{C}(V)) \]
First, we note that since neither $h$ or $f_{C}$ depends on $V$, and $f_C$ is a order preserving operator over $V$, we can take the maximization over $V$ directly to within $f_C$. 
\[\alpha = h\circ f_{C}\Big(\argmax_{V\in\mc{V}}h(V)\Big)\]
Let $V^\star = \argmax_{V\in\mc{V}}h_j(V)$. Then because $h$ does not involve $C$, we can take the maximization over $\Gamma$ directly in $f_C$.  
Let $C^\star = \argmax_{C \in \Gamma} h_j(f_C(V^\star))$ ,
\[\alpha_j = h_j\Big( f_{C^\star}(V^\star)\Big)\]
\end{proof}




==> intervalEx.tex <==
\section{Interval-based Bellman Operator}
\label{sec:ex}

Next, we consider an uncertainty set $\mc{C}$ described by intervals. In this case we can exactly bound sets $F_{\mc{C}}(V_0)$ and $\mc{V}^\star$. Suppose the uncertainty set $\mc{C}$ is given by 
\begin{equation}\label{eqn:intervalC}
\mc{C} = \Big\{C \in \reals^{S\times A} \ | \ C_{sa} \in [\underline{C}_{sa}, \overline{C}_{sa}], \ \forall\ (s,a) \in [S]\times[A] \Big\}.
\end{equation}
and the input value function set is given by 
\begin{equation}\label{eqn:invervalV}
\mc{V} = \Big\{V \in \reals^{S} \ | \ V_s \in [\underline{V}_{s}, \overline{V}_{s}], \ \forall\ s \in [S]\Big\}.
\end{equation}
We first show that the Hausdorff distance between two interval sets $\mc{V}, \mc{V}' \in \ H(\reals^S)$ can be computed by only comparing the upper and lower bounds of the interval themselves. 
\begin{lem}\label{lem:intervalHausdorff}
For two intervals $\mc{X}, \mc{Y} \in H(\reals^S, \norm{\cdot}_\infty)$ given by $\mc{X} = \intervalSet{x}$, $\mc{Y} = \intervalSet{y}$, where $\underline{x}, \overline{x}, \underline{y}, \overline{y} \in \reals^S$, their Hausdorff distance can be calculated as 
\[d_H(\mc{X},\mc{Y}) = \max\{\norm{\underline{x} - \underline{y}}_\infty, \norm{\overline{x} - \overline{y}}_\infty\}\]
\end{lem}
\begin{pf}
We consider the Hausdorff distance for the scalar case by noting that the infinity norm on $\reals^S$ has the property~\citep{chavent2004hausdorff}
\[d_H(\mc{X}, \mc{Y}) = \max_{i \in [S]} \ d_H(\mc{X}_i, \mc{Y}_i),\]
where $\mc{X} = \mc{X}_1\times\ldots\mc{X}_S$ and $\mc{Y} = \mc{X}_1\times\ldots\mc{X}_S$. On $(\mc{X}_i, \mc{Y}_i)$, we represent the intervals by $\mc{X}_i  = [\underline{x_i}, \overline{x_i}]$ and $\mc{Y}_i  = [\underline{y_i}, \overline{y_i}]$. 
Suppose the boundary points satisfy $\underline{x_i} \leq \overline{x_i} < \underline{y_i} \leq \overline{y_i}$, then for a fixed point $x_i \in \mc{X}_i$, $\inf_{y_i \in \mc{Y}_i}\norm{x_i - y_i}_\infty = \norm{x_i - \underline{y}_i}_\infty$. Since $x_i \in \intervalSet{x_i}$, the supremum over $\mc{X}_i$ of all possible $\norm{x_i - \underline{y_i}}_\infty$ is $\norm{\underline{x_i} - \underline{y_i}}_\infty$. Similarly, for a fixed point $y_i \in \mc{Y}_i$, $\inf_{x_i \in \mc{X}_i}\norm{x_i - y_i}_\infty = \norm{\overline{x_i} - y_i}_\infty$, taking the supremum over $\mc{Y}_i$ of all possible $\norm{\overline{x_i} - y_i}$ gives $\norm{\overline{x_i} - \overline{y_i}}_\infty$. Therefore, 
\begin{equation}\label{eqn:componentHausdorff}
  d_H(\mc{X}_i, \mc{Y}_i) = \max\{\norm{\underline{x_i} - \underline{y_i}}_\infty, \norm{\overline{x_i} - \overline{y_i}}_\infty\}.   
\end{equation}
We have shown this for the particular cases that $\underline{x_i} \leq \overline{x_i} < \underline{y_i} \leq \overline{y_i}$. It can be checked that~\eqref{eqn:componentHausdorff} is also satisfied for all other cases of order between  $\underline{y_i}, \underline{x_i},  \overline{x_i}, \overline{y_i} \in \reals$. Then the total Hausdorff distance between $\mc{X}$ and $\mc{Y}$ is given by 
\begin{equation}
    \begin{aligned}
        d_H(\mc{X}, \mc{Y}) & = \underset{i \in [S]}{\max} \{ \max\{\norm{\underline{x_i} - \underline{y_i}}_\infty, \norm{\overline{x_i} - \overline{y_i}}_\infty\} \} \\
        & = \max\{\norm{\underline{x} - \underline{y}}_\infty, \norm{\overline{x} - \overline{y}}_\infty\}
    \end{aligned}
\end{equation}
\end{pf}
Lemma~\ref{lem:intervalHausdorff} shows that interval sets are \emph{nice} in that its set-based Hausdorff distance can be derived by computing the element-based operations on the boundaries of the interval. We wish to show that similarly, set-based Bellman operator with interval sets can be solved by iterating over the boundary points of the uncertainty interval with operator $f_{C}$. To do so we utilize interval arithmetics to relate element-wise operations and set-based operations. 
\begin{equation}\label{eqn:intervalArith}
    \begin{aligned}
        \alpha[a,b] & = [\alpha a, \alpha b], \quad \alpha \geq 0 ,\\
        [a, b] + [c, d] & = [a + c, b + d], \\
        [a, b] - [c, d] & = [a - c, b - d], \\
        \min\{[a, b], [c, d]\} &  = [\min\{a, c\}, \min\{b, d\}],
    \end{aligned}
\end{equation}
where the last operator $\min\{[a,b], [c,d]\}$ denotes the smallest interval that contains $\{ \min\{x,y\}, | \ x \in [a,b], y \in [c,d]\}$. The equivalence relationship for the $\min$ operator is not as obvious as standard addition and subtraction. Here we prove that the equivalence for $\min$ operator is indeed as given. 
% To derive an expression for $F_{\mc{C}}(\mc{V})$ when $\mc{C}$ is an interval given. We utilize the following interval set-based arithmetic given in~\eqref{eqn:intervalArith}. 
% While the addition and subtraction operators for interval sets are standard, the $\min$ operator is not so obviously. We show here that the minimizing operator holds here.
% \tc{blue}{I do not understand the meaning of the $\min\{[a,b];[c,d]\}$. This does not correspond to intersection and neither to the union of intervals. Can you provide an example? }
% \tc{blue}{Do you mean that $\min\{[a,b],[c,d]\}$ is the smallest interval that contains $\{\min\{x,y\},x\in [a,b], y\in [c,d]\}$? } 

\begin{lem}\label{lem:minSetOperator}
The $\min$ operator for intervals can be calculated as 
\[ \min\{[a, b], [c, d]\}   = [\min\{a, c\}, \min\{b, d\}]\]
\end{lem}
\begin{pf}
Let the two sets be $\mc{A} = \min\{[a, b], [c, d]\}$ and $\mc{B} = [ \min\{a, c\}, \min\{\ b, d\} ]$, we first show that $\mc{A} \subseteq \mc{B}$. For $z \in \min\{[a, b], [c, d]\}$, there exists $x \in [a,b]$ and $y \in [c,d]$ such that $z = \min\{x,y\}$. Then necessarily, $\min\{a,c\} \leq z$ and $z \leq \min\{b,d\}$ must be satisfied. 

To see the inclusion $\mc{B} \subseteq \mc{A}$ is also true, take $v \in [\min\{a, c\}, \min\{b, d\}]$.  If $v \in [a,b]$, then $v  = \min \{ v, \max \{ v, d \} \}$. If $\max\{v,d\} = d$, $d \in [c,d]$, and so $v \in\min\{[a, b], [c, d] \}$. If $\max\{v,d\} = v$, then $d < v \leq b$, then this contradicts $v \in [\min\{a, c\}, \min\{b, d\}]$. 

If $v \notin [a,b]$, then either $c \leq v < a$ or $b < v \leq d$. $b < v \leq d$ cannot be true since $v \in [\min\{a, c\}, \min\{b, d\}]$. 
$c \leq v < a$ implies that $v \in [c,d]$ and $v = \min\{v, a\}$, then $v \in \min\{[a, b], [c, d] \}$.
\end{pf}
\begin{prop}
For interval sets $\mc{C}$ and $\mc{V}$ given by~\eqref{eqn:intervalC} and~\eqref{eqn:invervalV}, respectively, set-based Bellman operation is given by 
$F_{\mc{C}}(\mc{V}) = \{V \ | \ V \leq V_u, \ -V \leq V_l, \ V \in \reals^{S}\}$, where $V_l = f_{\underline{C}}(\underline{V})$ and $V_u = f_{\overline{C}}(\overline{V})$. 

Furthermore, we consider the sequence $\{\mc{V}_k\}$ generated by $\mc{V}^{k+1} = F_{\mc{C}}(\mc{V}^k)$, then we have that 
\[d_H(\mc{V}^k, \mc{V}^\star) \leq \epsilon/2\]
where $\epsilon > d_H(\mc{V}^{k}, \mc{V}^{k-1})\frac{2\gamma}{1 - \gamma}$. 
\end{prop}
\begin{pf}
The set operator $F_{\mc{C}}(\mc{V})$ can be equivalently written component-wise as $ \min_{a \in[A]} \intervalSet{C_{sa}} + \gamma \sum_{s'} P_{s',sa}\intervalSet{V_{s}}$, where the intervals are closed by definition. To see this, note that from definition of $F_{\mc{C}}(\mc{V})$, it is the closure of the union of images $f_C(V)$ for all possible combinations of $(C, V) \in \mc{C} \times \mc{V}$. 

We wish to obtain a set $\Lambda$ such that $F_{\mc{C}}(\mc{V}) \subseteq \Lambda$. As it turns out, for the interval uncertainty case, we can \emph{exactly} characterize $F_{\mc{C}}(\mc{V})$. Suppose that we have interval sets $\mc{C}$, $\mc{V}$, then we can directly perform interval arithemtics component-wise for $F_{\mc{C}}$ as
\begin{equation}
    \begin{aligned}
         \Big(F_{\mc{C}}(\mc{V})\Big)_s & = \min_{a \in [A]} \intervalSet{C_{sa}} + \gamma\sum_{s'} P_{s',sa}\intervalSet{V_s} \\
         & = \min_{a \in [A]} \Big[\underline{C_{sa}} + \gamma\sum_{s'}P_{s',sa}\underline{V_s},\  \overline{C_{sa}} + P_{s',sa}\overline{V_s}\Big] \\
         & = \Big[\min_{a \in [A]}\underline{C_{sa}} + \gamma\sum_{s'}P_{s',sa}\underline{V_s}, \\
         &\quad \quad \min_{a \in [A]}\overline{C_{sa}} + \gamma\sum_{s'}P_{s',sa}\overline{V_s} \Big] \\
         & = [\Big(f_{\underline{C}}(\underline{V})\Big)_s, \ \Big(f_{\overline{C}}(\overline{V})\Big)_s] \\
    \end{aligned}
\end{equation}

Therefore the image of $F_{\mc{C}}$ is another closed interval. From Theorem~\ref{thm:uniqueSetFixedPont}, any $\mc{V}^0 \in H(\reals^S)$ generates a sequence $\mc{V}^{k+1} = \mc{V}^k$ which satisfies 
$\lim_{k \rightarrow} F_{\mc{C}}^k (\mc{V}^0) = \mc{V}^\star$. Taking the limit of $\lim_{k \rightarrow}F_{\mc{C}}^k$
Then we can use interval-based arithmetics to derive $\mc{V}^\star = \lim_{k\rightarrow \infty} F_{\mc{C}}(\mc{V}^k) = \Big[  \lim_{k\rightarrow \infty}f_{\underline{C}}^k(\underline{V}),  \lim_{k\rightarrow \infty}f_{\overline{C}}^k(\overline{V}) \Big] = \intervalSet{\mc{V}^\star}$,  
% \begin{equation}
% \begin{aligned}
% \mc{V}^\star & = \lim_{k\rightarrow \infty} F_{\mc{C}}(\mc{V}^k) \\
% & = \lim_{k\rightarrow \infty} [f_{\underline{C}}^k(\underline{V}), f_{\overline{C}}^k(\overline{V})] \\
% & = [\lim_{k\rightarrow \infty}f_{\underline{C}}^k(\underline{V}),  \lim_{k\rightarrow \infty}f_{\overline{C}}^k(\overline{V})] \\
% & = \intervalSet{\mc{V}^\star}
% \end{aligned}
% \end{equation}
where $\underline{\mc{V}^\star}$($\overline{\mc{V}^\star}$) the fixed point of $f_{\underline{C}}$($f_{\overline{C}}$). 

At each iteration, the Hausdorff distance between $\mc{V}^k$ and $\mc{V}^\star$ is given by $d_{H}(\mc{V}^k, \mc{V}^\star) = d_H\Big([f_{\underline{C}}^k(\underline{V}), f_{\overline{C}}^k(\overline{V})], \intervalSet{\mc{V}^\star}\Big)$.
% \begin{equation}
%     \begin{aligned}
%     d_{H}(\mc{V}^k, \mc{V}^\star) & = d_H\Big([f_{\underline{C}}^k(\underline{V}), f_{\overline{C}}^k(\overline{V})], \intervalSet{\mc{V}^\star}\Big)
%     \end{aligned}
% \end{equation}
Using Lemma~\ref{lem:intervalHausdorff}, $ d_{H}(\mc{V}^k, \mc{V}^\star)$ is an interval given by \[ \Big[ \norm{f_{\underline{C}}^k(\underline{V}) - \underline{\mc{V}^\star}}_\infty , \norm{f_{\overline{C}}^k(\overline{V}) - \overline{\mc{V}^\star}}_\infty \Big].\] Similarly, 
\begin{align*}
d_H(\mc{V}^{k+1}, \mc{V}^k)= \max\Big\{   \norm{f_{\underline{C}}^k(\underline{V}) - f_{\underline{C}}^{k+1}(\underline{V})}_\infty, \\
 \norm{f_{\overline{C}}^k(\overline{V}) - f_{\overline{C}}^{k+1}(\overline{V})}_\infty \Big\}.
\end{align*}
From Theorem~\ref{thm:stoppingCriteria}, if $\norm{f_{\underline{C}}^k(\underline{V}) -  f_{\underline{C}}^{k+1}(\underline{V})}_\infty  < \epsilon \frac{1 - \gamma}{2\gamma} $ for some $\epsilon > 0$, then $ \norm{f_{\underline{C}}^k(\underline{V}) - \underline{\mc{V}^\star}}_\infty < \frac{\epsilon}{2}$. Therefore if $d_H(\mc{V}^{k+1}, \mc{V}^k) < \frac{(1 - \gamma)\epsilon}{2\gamma}$, then $d_H(\mc{V}^{k+1} - \mc{V}^\star) < \frac{\epsilon}{2}$. 
\end{pf}

We note that while $\mc{V}^k$ converges to $\mc{V}^\star$ in the Hausdorff sense, it is not an over approximation to $\mc{V}^\star$. In fact, if $\underline{\mc{V}} > \underline{\mc{V}^\star}$, then each $\mc{V}^\star \subsetneq \mc{V}^k $ for all $k$. Nonetheless, we can still utilize $\mc{V}^k$ to obtain an \emph{over-approximation} of $\mc{V}^\star$ by using estimate intervals $\bar{\mc{V}}^{k+1} = [f_{\underline{C}}^k(\underline{V}) - \ones\epsilon, f_{\underline{C}}^k(\underline{V})+ \ones\epsilon]$. 

% and for each state action pair, the interval $h_{s}(V)$ is given by 
% \begin{equation}
% \begin{cases}
% h^+_{s}(V) = &V_{s} \\
% h^-_{s}(V) = &-V_{s} \\
% \end{cases}, \quad \forall \ s \in [S]
% \end{equation}
% Then from Theorem, $V^\star$ is exactly defined by the boundaries of $\mc{V}$, 
% \[V^\star = \begin{cases}
% \argmax_{V \in \mc{V}} h^+_{s}(V) & = \overline{V}_{s} \\
% \argmax_{V \in \mc{V}} h^-_{s}(V) & =  \underline{V}_{s}
% \end{cases}\]
% to determine $C^\star$, we consider component-wise operation of $f_C$, let $V^+ = f_C(V^\star)$, then 
% \[V^+_s = \min_{a} C_{sa} + \sum_{s'}P_{s'sa}V^\star_{s'}\]
% We analyze $h^+_s$ and $h^-_s$ separately. For $h^+_s$, 
% \[\alpha_s^+ = \argmax_{C \in \Gamma}\Big(\min_{a} C_{sa} + \sum_{s'}P_{s'sa}\overline{V}_{s'}\Big)\]
% Here 
% we note that because $f_C$ is order preserving, we can directly move $\argmax_{C \in \Gamma}$ to within the minimization over actions. 
% \begin{align}
% \argmax_{C \in \Gamma} V^+_s & = \min_{a} \argmax_{C\in\Gamma}\Big(C_{sa}\Big) + \sum_{s'}P_{s'sa}\overline{V}_{s'} \\
% & = \min_{a} \overline{C}_{sa} + \sum_{s'}P_{s'sa}\overline{V}_{s'}
% \end{align}

% For $h^-_{sa}$, we have
% \begin{align}
% \argmax_{C \in \Gamma} -\Big( \min_a C_{sa} + \sum_{s'}P_{s'sa}\underline{V}_{s'}\Big) \\
% \argmax_{C \in \Gamma} \Big( \max_{a} -C_{sa} - \sum_{s'}P_{s'sa}\underline{V}_{s'}\Big)
% \end{align}
% Here define $\tilde{f} = \max_a -C_{sa}$, then $\tilde{f}$ is an order \emph{reversing} operator. Therefore when taking the $\argmax_{C\in\Gamma}$ inside, we take the $\argmin$ instead. 
% \begin{align}
%     \alpha^-_s & = \max_a -\argmin_{C \in\Gamma}C_{sa} - \sum_{s'} P_{s'sa}\underline{V}_{s'} \\
%     & = \max_{a} - \underline{C}_{sa} - \sum_{s'}P_{s'sa}\underline{V}_{s'} \\ 
%     &  = \min_{a} \underline{C}_{sa} + \sum_{s'}P_{s'sa}\underline{V}_{s'}s
% \end{align}

% This shows that we can bound $F_{\mc{C}}(\mc{V})$ by iterating over the boundaries of both $\mc{V}$ and $\mc{C}$, i.e.
% \[\Lambda = \{V \in \reals^{S} \ | \ \begin{cases}
% V \leq f_{\overline{C}}(\overline{V}) \\
% -V \leq f_{\underline{C}}(\underline{V})
% \end{cases}\}\]
% Through Theorem 1 we've shown that $F_{\mc{V}}(\mc{V}) \subseteq \Lambda$, next we show that $\Lambda = F_{\mc{C}}(\mc{V})$.

% We note that the boundary points of $\Lambda$, $f_{\overline{C}}(\overline{V})$ and $f_{\underline{C}}(\underline{V})$, can be acheived through taking the appropriate cost from $\Gamma$ and value function from $\mc{V}$. Any $V' \in \Lambda$ can be written as 
% \[V'_s = (1 - \lambda_s)f_{\overline{C}}(\overline{V})_s + \lambda_s f_{\underline{C}}(\underline{V})_s, \quad \lambda_s \in (0,1) \]
% Using definition of $f_{C}$, 
% \[V'_s = \min_a (1 - \lambda_s)\overline{C}_{sa} + \lambda_s\underline{C}_{sa} + \sum_{s'}P_{s'sa}\Big((1-\lambda_s)\overline{V}_s + \lambda_s\underline{V}_s\Big)\]
% Since there exists $C \in \Gamma$ where for each state action pair, $C_{sa} = (1 - \lambda_s)\overline{C}_{sa} + \lambda_s\underline{C}_{sa}$, and there exists $V \in \mc{V}$ such that at each state $V =(1-\lambda_s)\overline{V}_s + \lambda_s\underline{V}_s $, we have that $V' \in F_{\mc{C}}(\mc{V})$. Therefore, $\Lambda \subseteq F_{\mc{C}}(\mc{V})$. 

% \begin{corollary}
% In the bounded intervals example given in Example~\ref{ex:intervalVI}, the set $\Lambda$ exactly bounds 
% \end{corollary}
% \begin{proof}
% See Example~\ref{ex:intervalVI}. 
% % We use  interval arithmetic to show this. Here are some interval arithmetic operations defined. 
% % \begin{subequations}
% % \begin{align}
% %     [a,b] + [c,d] & = [a+c, b+d] \\
% %     [a,b] - [c,d] & = [a-c, b-d] \\
% %     \min\{[a,b], [c,d]\} & = [\min\{a,c\}, \min\{b,d\}]
% % \end{align}
% % \end{subequations}
% % \ForAuthorsAssa{The operation of min is standard? A short explanation should be added to avoid confusion with the intersection/union operator. For example, $x\in \min\{[a,b],[c,d]\}$ iff $\min{a,c}\leq x\leq \min{b,d}$. For me, the min operator on intervals corresponds to intersection....}
% % Let $V_0 = 0$, then $V_1$ is
% % \begin{align}
% % V_1(s) & = \min_{a \in [A]} \{[\underline{C}_{sa}, \overline{C}_{sa}] \}\\
% % & = [\min_{a}\{\underline{C}_{sa}\}, \min_a \{\overline{C}_{sa}\}]
% % & = [\underline{V}_1(s), \overline{V}_1(s)]
% % \end{align}
% % where we call this new upper and lower bound $\underline{V}$ and $\overline{V}$. 

% % Iterating the next step, we obtain
% % \begin{align}
% % V_2(s) & = \min_a\{[\underline{C}_{sa}, \overline{C}_{sa}] + \sum_{s'}P_{ss'a}[\underline{V}_1(s), \overline{V}_1(s)]\}
% % \end{align}
% % For each state action pair, the interval sum becomes 
% % \[[\underline{C}_{sa} + \sum_{s'}P_{ss'a}\underline{V}_1(s), \overline{C}_{sa} + \sum_{s'}P_{ss'a}\overline{V}_1(s)]\]
% % Then the value function at the next time step becomes 
% % \[\min_{a}\{\underline{C}_{sa} + \sum_{s'}P_{ss'a}\underline{V}_1(s)\}, \min_a \{\overline{C}_{sa} + \sum_{s'}P_{ss'a}\overline{V}_1(s)\}\]
% % Let the new upper and lower bounds be $\underline{V}_2(s)$ and $\overline{V}_2(s)$. Then we observe that if $\underline{V}_1$ and $\overline{V}_1$ are the value functions iterated once over $\underline{C}$ and $\overline{C}$, the resulting $\underline{V}$ and $\overline{V}$ are then also the value functions iterated twice over $\underline{C}$ and $\overline{C}$. Then we obtain that at each step, value iteration over the set $[\underline{C}, \overline{C}]$ satisfies
% % \[V_k \in [\underline{V}_k, \overline{V}_k],\]
% % if $\underline{V}_k$ is the $k$-th iteration over cost function $\underline{C}$, and $\overline{V}_k$ is the $k$-th iteration over cost function $\overline{C}$. 

% % Suppose that the value iteration converges to an optimal value function $\lim_kV_k = V^\star$, then $V^\star$ is necessarily bounded by 
% % \[V^\star = [\underline{V}, \overline{V}],\]
% % where $\underline{V} = \lim_{k\rightarrow\infty}\underline{V}$ and $\overline{V} = \lim_{k\rightarrow\infty}\overline{V}_k$ --- i.e. the optimal value function of costs $\underline{C}$ and $\overline{C}$. 

% % However, note that at each iteration, $[\underline{V}_k, \overline{V}_k]$ does not necessarily bound $[\underline{V}, \overline{V}]$. In fact, because single cost value iteration always over approximates the value function, $\underline{V}_k$ is always above $\underline{V}$. 

% % To resolve this, we utilize the stopping criteria. 
% % \begin{theorem}
% % At each iteration, let $\epsilon_k = \norm{V_{k+1} - V_{k}}\frac{2\gamma}{1 - \gamma}$, then we have an over approximation to $\mc{V}^\infty$ at each step $k$: 
% % \[\mc{V}^\infty \in [\underline{V}_k - \epsilon_k, \overline{V}_k]\]
% % \end{theorem}
% \end{proof}


% With out loss of generality, we can consider the initial set $V_0$ to be a singleton, since the propagation of $V_0\times \mc{C}$ results in a set value $F(V_0, \mc{C})$. We define $\Lambda^N$ as the image of set $(V_0, \mc{C})$ after $N$ iterations of $F$, formally as 
% \begin{equation}
% \Lambda^N(\mc{C}) = \{V^{N+1} \ | \ \exists \{C_k\}_0^N \subseteq \mc{C}, \ V_{k+1} = F(V_k, C_k), \ \forall k \in [N\}. 
% \end{equation}
% The limit of $\Lambda^N$ is denoted as $\Lambda^\infty = \lim_{N \rightarrow \infty} \Lambda_N$

% For any input set $\Gamma$, we consider estimating the resulting value function invariant set by $\Tilde{\Lambda}$, defined by the sublevel set $\Tilde{\Lambda}  = \{V \ | \ h(V) \leq \alpha_v\}$. To obtain a meaningful characterization, we wish to minimize $\alpha_v$ such that the resulting set closely approximates $\Lambda^\infty$. 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> paperReview.tex <==
\section{Related Work}
\label{sec:relatedWorks}
Bounding the fixed point of the Bellman operator is related to robust MDP analysis~\citep{wiesemann2013robust}, where a minimax bound is given by considering MDP as a game between a minimizing and maximizing player, and assuming the problem parameters come from stochastic distributions. 
However, none of these works provide a systematic approach to bound the fixed point of a Bellman operator for a given set of MDP problems. 

The game model we consider in particular is a stochastic game first introduced by~\cite{shapley1953stochastic}. Learning algorithms that utilize Bellman type relationships are shown to be convergent in~\cite{hansen2013strategy} for policy iteration, and in~\cite{kearns2000fast} for value iteration. However, we have not seen any analysis of the effect of data parameter uncertainty on the learning dynamics of stochastic games.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> samePolicy.tex <==
\section{effects of cost uncertainty on policy}
\tc{red}{This is migrating to another overleaf soon}
Often in MDP related problems, we ask the following question: given a cost $C$, determine the set of optimal policies. However a reverse question can also be interesting: given a policy, what is the set of corresponding costs for which the policy is optimal? This is a more difficult question for two reasons. The first difficulty is determining a single cost for which a given policy is optimal. This is not a well examined problem so far. The second is determining a set of costs around this single cost that still guarantees optimality of the given policy. We show here that this can be addressed by utilizing our problem set up. Formally, the problem we attempt to solve is: given an uncertainty range around a cost for which a policy is optimal, how can we determine if the policy is optimal for the entire set of possible costs? 

\begin{theorem}
Given uncertainty cost interval $[\underline{C}, \overline{C}]$, if a policy $\pi$ is optimal for both the MDP defined by $\underline{C}$ and $\overline{C}$, then it is optimal for all MDP's corresponding to any cost $C\in [\underline{C}, \overline{C}]$. 
\end{theorem}
\begin{proof}
Suppose that $\pi$ is optimal for the MDP's defined for $\underline{C}$ and $\overline{C}$. Then we have that 
\[\underline{V} = (I - \gamma P\pi^T)^{-1}\underline{C},\  \overline{V} = (I - \gamma P\pi^T)^{-1}\overline{C}\]
For an element $C \in [\underline{C}, \overline{C}]$, we have that the corresponding optimal value function satisfies
\[ V = \min_{\pi \in \Pi} (I - P\pi^T)^{-1}C\pi^T \]
First we note that taking the minimum of a finite number of convex functions is a convex operation.\tc{red}{Is this $(I - P\pi^T)^{-1}C\pi^T$ convex?? yes it is, taking $C$ as the variable} 
Let the operation be defined by $p(C)$. Since $C_{s\pi(s)} \in [\underline{C}_{s\pi(s)}, \overline{C}_{s\pi(s)}]$, we have that 
\begin{align}
f(C) &\geq (1 - \lambda)f(\overline{C}) + \lambda f(\underline{C}) \\
& \geq (1 - \lambda)(I - \gamma P\pi^T)^{-1}\overline{C}\pi^T + \lambda (I - \gamma P\pi^T)^{-1}\underline{C}\pi^T \\
\min_{\pi \in \Pi} (I - \gamma P\pi^T)^{-1}C\pi^T & \geq (I - \gamma P\pi^T)^{-1}((1 - \lambda)\overline{C} + \lambda \underline{C})\pi^T \\
\min_{\pi \in \Pi} (I - \gamma P\pi^T)^{-1}C\pi^T & \geq (I - \gamma P\pi^T)^{-1}C\pi^T
\end{align}
Therefore, we see that $\pi$ minimizes the set of possible stationary value functions. We conclude that $\pi$ is optimal for any cost function $C \in [\underline{C}, \overline{C}]$ 

\end{proof}

==> stochasticGame.tex <==
\section{Bounding Values of a Stochastic Game}
\label{sec:stochasticGames}
% \ForAuthorsAssa{Perfect Information? With perfect information, we could use stationary and pure strategies. Without we have to use stationary mixed strategies.}
Our analysis of set-based Bellman operator is motivated by dynamic programming based learning algorithms in stochastic games. In this section, we apply bounded value iteration analysis to value iteration in a two player zero-sum stochastic game, and show that both transient and asymptotic behaviours of a player's value function can be bounded, regardless of how the opponent's strategy is updated. 
\subsection{Stochastic games}
Stochastic game extends a standard MDP to a multi-agent competitive setting~\citep{shapley1953stochastic}. In a stochastic game, $N$ players each solves its own MDP problem, where the $i^{th}$ player's MDP is given by $([S_i],[A_i],P_i,C_i, \gamma_i)$. However, as opposed to standard MDPs, the cost and and transition probabilities $C_i$ and $P_i$ of each player is a function of the \emph{joint strategy} of all players, denoted by $\pi = (\pi_1, \ldots, \pi_N)$, where $\pi_i$ is the strategy of the $i^{th}$ player. Therefore, stochastic game extends MDPs in the sense that the \emph{constant environment} defined in an MDP will become dependent on other players' strategies. 

Because the environment is varying, the usual notion of optimality in MDP must be expanded to reflect dependency of a player's optimal strategy on the joint strategy space. We consider a \emph{Nash equilibrium} in terms of the strategies of individual players~\citep{littman1994markov,littman2001value}. A Nash equilibrium policy always exists for a stochastic game~\citep{filar2012competitive}.
\begin{definition}[Nash Equilibrium]
A set of joint strategies $\pi^\star = \{\pi^\star_1, \ldots, \pi^\star_N\}$ is a Nash equilibrium if each policy is the fixed point of the Bellman operator,
\[V_i^\star = \Big(CM_{\pi^\star_i}^T + \gamma(V^\star_i)^TPM^T_{\pi_i^\star}\Big), \forall \ i \in [N].\]
\end{definition}
We consider a two player zero sum stochastic game, where each player solves a discounted MDP given by $( [S],[A], \gamma, P, C_{1,2} (\pi_1, \pi_2) ) $. Both players share an identical state-action space $([S],[A])$ as well as the same transition probabilities $P$. However, each player's cost is given by function $C_{1,2}: \reals^{2(S\times A)} \rightarrow \reals^{S\times A}$ that depends on both player's strategies. Player $1$'s cost is given by
\[C_1(\pi_1, \pi_2) = C_{sa} + A_{sa}\pi_2(s,a),  \quad A \in \reals_+^{(S\times A)},\]
while player $2$'s cost is given by 
\[C_2(\pi_1, \pi_2) = C_{sa} - A_{sa}\pi_1(s,a),  \quad A \in \reals_+^{(S\times A)},\]
where the matrix $A$ is the same for the two costs. Such a game is a zero sum minimax stochastic game~\citep{basar1999dynamic}. Under the minimax set up, a stationary deterministic policy always exists and will be reached when both players perform value iteration~\citep{littman1994markov} or variants of value iteration in the online setting, as shown in numerous works in multi-agent reinforcement learning~\citep{hu2003nash, littman2001value}. 

Although convergent algorithms exist, almost all of the existing work require that the players utilize specific rules to update their strategy. When players cannot coordinate their method of update, it is not true they will converge to a Nash equilibrium in general. In this section, we utilize our set-based Bellman operator to show that, although we cannot guarantee convergence of value iteration the exact trajectory of our player's minimizing trajectory, we can show instead that we can determine the invariant set which our player's value function converges to, \emph{despite} whatever the opponent is doing. 
% \subsection{Simulation model}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\columnwidth]{fig/MDP_ex.png}
%     \caption{To be changed}
%     \label{fig:grid_MDP}
% \end{figure}

We define the state space of a stochastic game on a $3\times 3$ grid,
%  shown in Fig~\ref{fig:grid_MDP}, 
where $S = 9$ and $A = 4$. From each state, the actions available are `left', `right', `up', or `down'. At each state $s$, the action `left' corresponds to the probability distribution where $p = 0.7$ to reach the state left of $s$, and $p = 0.1$ to reach the states right, below, and above state $s$, i.e. the neighbour states. The other three actions are similarly defined, with the most probability attributed in the direction of action, and a small probability of reaching other neighbouring states. From states where a particular action $a$ is not available --- e.g. the action `left' from a state on the left boundary of the grid --- taking $a$ corresponds to reaching one of the available neighbouring states with uniform probability distribution. 

On this state-action space, we initialize the cost $C$ as a random matrix, such that each entry $C_{sa} \in [0,1]$. The matrix $A$ is also randomly initialized, such that each $A_{sa} \in [0,0.1]$. This allows us to derive an interval-based cost uncertainty~\eqref{eqn:intervalC}, where 
\[(C_1)_{sa} \in [C_{sa}, C_{sa} + A_{sa}], \quad (C_2)_{sa} \in [C_{sa}, C_{sa} - A_{sa}]\]
The upper bounds for both intervals are achieved when the opponent's probability of taking action $a$ from state $s$ is $1$. We use this uncertainty to represent the cost that player $1$ and $2$ receive, regardless of which policy the opponent chooses. 

We consider a generic value iteration algorithm which is the basis for many dynamic programming based iterative solutions to stochastic games~\citep{filar2012competitive, littman1994markov}, in which player $1$ always performs a value iteration step that is the best response to its current value function, and chooses its optimal strategy as the best response, and player 2 obtains its optimal policy using some function $g: (\pi_1) \rightarrow \pi_2$, we do not make any assumptions of $g$, it can produce any general policy in response to the policy $\pi_1$. 
\begin{algorithm}
\caption{Two player VI}
\begin{algorithmic}[h]
\Require \((S,A,\gamma, P,C_{1,2})\), \(V_0\).
\Ensure \( V^\star, \pi^\star_1, \pi^\star_2\)
\State{\(\pi^x_0 = [0, \ldots , 0]\), \(\pi^y_0 = [0, \ldots , 0]\)}
\For{\(k = 0, \ldots, \)}
\State{\(C^k = C(\pi^k_1, \pi^k_2)\)}
\State{\(V^{k+1} = f_{C^k}(V^k))\)}
\State{\(\pi^{k+1}_1 = f_{C^k}(V^k)\)}
\State{\(\pi^{k+1}_2 = g(\pi^{k+1}_1) \)}
\EndFor % \For{\(t=T-1, T-2, \ldots, 0\)}
\end{algorithmic}
\label{alg:VI_stochasticGames}
\end{algorithm}

Algorithm~\ref{alg:VI_stochasticGames} in the online setting is also related to Q-learning for MARL~\citep{littman1994markov}. When both players update their strategies with a determined update rule, conditions which guarantee convergence towards Nash equilibrium is given in~\cite{littman1994markov, filar2012competitive,hansen2013strategy}. Our analysis provides bounds on player $1$'s value function when we do not know how player $2$ is updating its strategy. 


\subsection{Simulated results}
We first consider situations where both players are updating their strategies via value iteration utilizing the same state-action space, as well as probability kernel. Player $1$ is updating with a discount factor of $\gamma_1 = 0.7$, while player $2$ updates its policy with $\gamma \in [0,1]$. Assuming both players' value functions are initialized to be $0$, we simulate player $1$'s value function trajectories for different values of $\gamma$ in Figure~\ref{fig:discountFactor_VI}. 
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.04\columnwidth]{fig/T_50_gammaVarying.pdf}
    \caption{Player $1$'s value function as a function of state at different iterations $k = \{1, 49, 99\}$. The blue bounds show predicted interval $\mc{V} = [\underline{V}, \overline{V}]$. }
    \label{fig:discountFactor_VI}
\end{figure}

Figure~\ref{fig:discountFactor_VI} shows that when player $2$ utilizes different discount factors, player $1$ experiences \emph{different} trajectories despite the fact that both players are utilizing value iteration to minimize their losses. However, the value function trajectory that player $1$ follows is always bounded between the thresholds we derived from Proposition~\ref{prop:setConverge}. As Figure~\ref{fig:discountFactor_VI} shows, there does not seem to be any direct correlation between player $2$'s discount factor and player $1$'s value function. However, the interval bounds we derived do tightly approximate resulting value function trajectories.

Alternatively, suppose we know that player $2$ has the same discount factor as player $1$, but we do not know how it is updating its strategy nor its initial value function. 
We consider two extreme scenarios: when player $2$ is also minimizing its cost and when player $2$ is maximizing its cost. In Figure~\ref{fig:maxVsMin}, the infinity norm of player $1$'s value function at each iteration $k$ is shown with respect to these two scenarios. Both player $1$ and player $2$'s initial value function is randomly initialized for some $V_0(s) \in [0,1]$, $\forall \ s \in [S]$. The dotted trajectories are when player $2$ is also minimizing its own value function, while the solid trajectories are when player $2$ is maximizing its own value function. The grey box region shows the predicted norm bounds as derived from Proposition~\ref{prop:setConverge}. 
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{fig/VI_differentAlgs4.pdf}
    \caption{The infinity norm of player $1$'s value functions at each iteration $k$. }
    \label{fig:maxVsMin}
\end{figure}

The effect of player $2$'s strategy change caused a significant shift in player $1$'s value function trajectory. When the opponent player is attempting to maximize its own cost function, player $1$'s function achieves the absolute lower bound as predicted by Proposition~\ref{prop:BellmanCompact}. This is due to the fact that multiple actions with different costs is available at each state. Since both players are selecting from the set of deterministic policies $\Pi_d$, they are bound to select different actions unless all actions have the exact same cost. On the contrary, if player $2$ is also attempting to minimize its value function, then player $1$ and player $2$ would precisely select the same state-actions at every time step. Then depending on the coupling coefficient $A_{sa}$, they may or may not choose a less costly action at the next step. This causes both the high value cost and the limit cycle behaviour that the dotted trajectories displace. We note that Figure~\ref{fig:maxVsMin} also shows the bounds determined by set-based value iteration are fairly tight with respect to actual trajectories that the player may take. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> summary.tex <==
\newpage
\appendix
\section{Summary}
current structure
\begin{enumerate}
    \item[3] MDP and Bellman op
    \begin{enumerate}
        \item[] def of MDP, policy
        \item[] discounted infinite horizon expected cost
        \item[A] Bellman operator
        \begin{enumerate}
            \item[] Bellman op 
            \item[] \textbf{Def 1} : Fixpoint
            \item[] \textbf{Thm1}: existence of the fixpoint 
        \end{enumerate}
        \item[B] Termination criteria for value iteration
        \begin{enumerate}
            \item[] \textbf{Thm 2}: convergence of VI
        \end{enumerate}
    \end{enumerate}
    
    \item[4] Set-based value iteration
    \begin{enumerate}
    \item[] Haussdorf distance btw sets
    \item[] \textbf{Thm3} Haussdorf metric space of a complete metric space (cms) is a cms
    \item[] \textbf{Prop1}: when C compact, $F_C(V)$ in the same cms as V
    \item[] \textbf{Def2} Lower/Upper semi-continuous func
    \item[] \textbf{Lemma 1}: inf+closure on lower semi-cont. func
    \item[] \textbf{Lemma 2}: sup-inf + closure
    \item [] \textbf{Prop2}: $F_C$ is order preserving+contracting
    \item [] \textbf{Def3}: order preserving
    \item[] \textbf{Def4}: contracting
    \item [] \textbf{Prop 3}: banach fixpoint thm on cms
    \item [] \textbf{Def5}: set-based fixpoint (and $\bar{V}$)
    \item[A] Bounding value approx
        \begin{enumerate}
            \item[] template abstraction
            \item[] \textbf{Prop4}: tight abstraction
            \item[] \textbf{Thm4}: characterization of template bounds on order preserving functions
            \item[] \textbf{Example 1}: interval templates
            \item [] \textbf{Corollary 1}: ??? don't understand what it means
        \end{enumerate}
    \end{enumerate}
    \item[5] Bounding values on stochastic game
    \begin{enumerate}
        \item[A] Stochastic game
        \item[B] Grid MDP
        \item[C] Algorithms
        
    \end{enumerate}
\end{enumerate}
\newpage 
~\\
proposed structure
\begin{enumerate}
    \item[3] MDP and Bellman op\\
    BASIC DEFINITIONS: NO MENTION OF SETS YET
    \begin{enumerate}
        \item[A] MDP and optimal value
        \begin{enumerate}
        \item[] \textbf{Def}: def of MDP, policy
        \item[] \textbf{Def}: discounted infinite horizon expected cost
        \end{enumerate}
        \item[B] Bellman operator fixpoint: optimal value
        \begin{enumerate}
            \item[] \textbf{Def}: Bellman op 
            \item[] \textbf{Def 1} : Fixpoint
            \item[] \textbf{Thm1}: existence of the fixpoint 
        \end{enumerate}
        \item[C] Effective computation using value iteration, Termination criteria
        \begin{enumerate}
            \item[] \textbf{Thm 2}: convergence of VI
        \end{enumerate}
    \end{enumerate}
    
    \item[4] Set-based value iteration\\
    HERE WE DEFINE THE EXTENSION TO SETS AND ARGUE ABOUT THE EXISTENCE OF THE FIXPOINT OF THE LIFT OF BELMANN TO SETS
    \begin{enumerate}
    \item[] \textbf{Def}: Haussdorf distance btw sets
    \item[] \textbf{Thm3} Haussdorf metric space of a complete metric space (cms) is a cms
    \item[] \textbf{Prop1}: when C compact, $F_C(V)$ in the same cms as V
    \item[] \textbf{Def2} Lower/Upper semi-continuous func
    \item[] \textbf{Lemma 1}: inf+closure on lower semi-cont. func
    \item[] \textbf{Lemma 2}: sup-inf + closure
    \item [] \textbf{Def3}: order preserving
    \item[] \textbf{Def4}: contracting
    \item [] \textbf{Prop2}: $F_C$ is order preserving+contracting
    \item [] \textbf{Prop 3}: banach fixpoint thm on cms
    \item [] \textbf{Def5}: set-based fixpoint (and $\bar{V}$)
    \end{enumerate}
    
    \item[5] Template-based abstraction of set-based value iteration\\
    TODO: REDEFINE THE SET EXTENSION OF MDP WITH THE FUNCTION g(C) AND THE TEMPLATE h
        \begin{enumerate}
            \item[] \textbf{Def}: template abstraction, introduce the bounds more formally. 
            \item[] \textbf{Prop4}: tight abstraction
            \item[] \textbf{Thm4}: characterization of template bounds on order preserving functions\\
            here $\tilde{\Lambda}$ is mentioned but never used, you implicitly assume it is related to $\alpha_v$ 
        \end{enumerate}
    \item[6] Example\\
    COULD YOU PROVIDE TWO INSTANCIATIONS FOR h, ONE WITH INTERVAL TEMPLATES AND ONE WITH ANOTHER LINEAR RELATIONSHIP OR A QUADRATIC ONE?
    \begin{enumerate}
                \item[] \textbf{Example 1}: interval templates
            \item [] \textbf{Corollary 1}: ??? don't understand what it means
    \end{enumerate}

    \item[7] Bounding values on stochastic game
    \begin{enumerate}
        \item[A] Stochastic game
        \item[B] Grid MDP
        \item[C] Algorithms
        
    \end{enumerate}
    \end{enumerate}
    
